Comparative evaluation of bandwidth-bound applications on the Intel Xeon CPU MAX Series

In this paper we explore the performance of Intel Xeon MAX CPU Series, representing the most significant new variation upon the classical CPU architecture since the Intel Xeon Phi Processor. Given the availability of a large on-package high-bandwidth memory, the bandwidth-to-compute ratio has significantly shifted compared to other CPUs on the market. Since a large fraction of HPC workloads are sensitive to the available bandwidth, we explore how this architecture performs on a selection of HPC proxies and applications that are mostly sensitive to bandwidth, and how it compares to the previous 3rd generation Intel Xeon Scalable processors (codenamed Ice Lake) and an AMD EPYC 7003 Series Processor with 3D V-Cache Technology (codenamed Milan-X). We explore performance with different parallel implementations (MPI, MPI+OpenMP, MPI+SYCL), compiled with different compilers and flags, and executed with or without hyperthreading. We show how performance bottlenecks are shifted from bandwidth to communication latencies for some applications, and demonstrate speedups compared to the previous generation between 2.0x-4.3x.

==> artifact.tex <==
Abstract

The paper entitled "Comparative evaluation of bandwidth-bound applications on the Intel Xeon CPU MAX Series" performs the detailed benchmarking of a number of computational science applications and proxies in Intel's Xeon CPU MAX 9480 CPUs, and compares them to eariler Intel CPUs (Xeon 8360Y) and AMD CPUs (EPYC 7V73X), using a range of different parallelizations and compilers.

As such, the contributions of the paper rely entirely on computational results - specifically performance measurements. All measurements are reported automatically by the test framework, and are then parsed using scripts or by hand, and assembled into tables and figures shown in the paper. Most figures show runtimes, or normalized runtimes (i.e. speedups), which are derived trivially from the application logs. Figure 8 shows achieved bandwidth, which was calculated based on automated reporting for individual applications, accumulated with a weighted average.

The reproducibility of the results in the paper relies solely on the test framework available on GitHub (https://github.com/reguly/tests), which has been built to make it easy to run all experiments easily, producing application logs, which contain all the raw data for the results (runtimes, communication times, and bandwidth numbers).

Repro of experiments
The hardware and software environments are described in detail in the paper's Section 2.
To get and compile the test environment, take the following steps:
%START_LATEX
\begin{enumerate}
\item \texttt{git clone --recursive https://github.com/reguly/tests.git}
\item To build dependent libraries, and download meshes, execute the \texttt{op2\_dependencies.sh} and \texttt{op2\_get\_data.sh} scripts in the root directory
\item edit the \texttt{source\_intel} and \texttt{source\_sycl} files to match your environment, and choice of compilers
\item execute the \texttt{build\_cpu.sh} script to build MPI and MPI+OpenMP versions of the applications
\item execute the \texttt{build\_sycl.sh} script to build the MPI+SYCL variants of the applications
\item edit and execute the \texttt{run\_all.sh} script to match your compiler and application types to be tested (CPUTEST and/or SYCL). Can use further command line parameters to run only a specific application
\item results are placed in log files named \texttt{*\_diag2}, these can be pulled into the current directory with e.g. \texttt{find ../../tests/ -name "*diag2" -exec mv \{\} ./ \\ ;}. Use the \texttt{parse.py} file, passing the name of the directory containing these gathered files to extract timing data into tables.
\item Figures can be generated using the heatmaps.ipynb, which reads in the test1.xlsx and results\_summary.xlsx files, which need to be populated with the tables from the previous step.
\end{enumerate}
%STOP_LATEX

Depending on the hardware platform, the compilation takes 1-5 minutes, and the execution of the full set of benchmarks takes between 20 mins and 1.5 hours.


It includes:
(i) a complete description of the experiment workflow that the computational artifact(s) can execute
(ii) an estimation of the execution time to execute the experiment workflow.
(iii) a complete description of the expected results and an evaluation of them, and most importantly.
(iv) how the expected results from the experiment workflow relate to the results found in the article. Best practices indicate that, to facilitate the understanding of the scope of the reproducibility, the expected results from the artifact should be in the same format as the ones in the article. For instance, when the results in the article are depicted in a graph figure, ideally, the execution of the code should provide a (similar) figure (there are open-source tools that can be used for that purpose such as gnuplot). It is critical that authors devote their efforts on these aspects of the reproducibility of experiments to minimize the time needed for their understanding and verification.
